Machine Learning-Driven Adaptive OpenMP For Portable Performance on Heterogeneous Systems

Heterogeneity has become a mainstream architecture design choice for building High Performance Computing systems. However, heterogeneity poses significant challenges for achieving performance portability of execution. Adapting a program to a new heterogeneous platform is laborious and requires developers to manually explore a vast space of execution parameters. To address those challenges, this paper proposes new extensions to OpenMP for autonomous, machine learning-driven adaptation. Our solution includes a set of novel language constructs, compiler transformations, and runtime support. We propose a producer-consumer pattern to flexibly define multiple, different variants of OpenMP code regions to enable adaptation. Those regions are transparently profiled at runtime to autonomously learn optimizing machine learning models that dynamically select the fastest variant. Our approach significantly reduces users' efforts of programming adaptive applications on heterogeneous architectures by leveraging machine learning techniques and code generation capabilities of OpenMP compilation. Using a complete reference implementation in Clang/LLVM we evaluate three use-cases of adaptive CPU-GPU execution. Experiments with HPC proxy applications and benchmarks demonstrate that the proposed adaptive OpenMP extensions automatically choose the best performing code variants for various adaptation possibilities, in several different heterogeneous platforms of CPUs and GPUs.

==> figures/adaptive_example_lowered.tex <==
\begin{minted}[linenos,frame=lines,fontsize=\scriptsize]{c++}
  Apollo::Region *region =  Apollo::instance()->getRegion(scoring-loop, 1,  3, 1);
  region->begin({(float)nDiag} ); 
  int policy = region->getPolicyIndex();
  
  if (policy ==2){
    #pragma omp target enter data map(to:a[0:m-1], b[0:n-1]) \ 
      map(to: H[0:asz], P[0:asz], maxPos)
  }
  
  for (i = 1; i <= nDiag; ++i) {
    switch (policy)    {
      case 0:  /* variant 0: serial */
        for (j = 0; j < nEle; ++j)
          similarityScore(si-j, sj+j, H, P, &maxPos); 
      case 1: /* variant 1: CPU threading */
        #pragma omp parallel for
        for (j = 0; j < nEle; ++j)
          similarityScore(si-j, sj+j, H, P, &maxPos); 
        break;
      case 2: /* variant 2: GPU offloading */
        #pragma omp target teams distribute parallel for map (...)
        for (j = 0; j < nEle; ++j)
          similarityScore(si-j, sj+j, H, P, &maxPos); 
        break;
      default:
         /* .. error handling here... */
    }  
  }
  
  if (policy ==2){
    #pragma omp target  target exit data map(from: H[0:asz], P[0:asz], maxPos)
  }
  region->end();
 \end{minted}
